CliniQG4QA: Generating Diverse Questions for Domain Adaptation of Clinical Question Answering

Clinical question answering (QA) aims to automatically answer questions from medical professionals based on clinical texts. Studies show that neural QA models trained on one corpus may not generalize well to new clinical texts from a different institute or a different patient group, where large-scale QA pairs are not readily available for model retraining. To address this challenge, we propose a simple yet effective framework, CliniQG4QA, which leverages question generation (QG) to synthesize QA pairs on new clinical contexts and boosts QA models without requiring manual annotations. In order to generate diverse types of questions that are essential for training QA models, we further introduce a seq2seq-based question phrase prediction (QPP) module that can be used together with most existing QG models to diversify the generation. Our comprehensive experiment results show that the QA corpus generated by our framework can improve QA models on the new contexts (up to 8% absolute gain in terms of Exact Match), and that the QPP module plays a crucial role in achieving the gain.

==> Tables/table2.tex <==
\begin{table*}[t]
\centering
\caption{Automatic evaluation of the generated questions on emrQA dataset. For each base model, the best performing variant is in \textbf{bold}.}
\label{tbl:qg_results}
\begin{tabular}{lcccc|cccc}
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{4}{c|}{\textbf{Relevance}} & \multicolumn{4}{c}{\textbf{Diversity}} \\ \cline{2-9} 
 & \textbf{BLEU3} & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE-L} & \textbf{Distinct3} & \textbf{Distinct4} & \textbf{Entropy3} & \textbf{Entropy4} \\ \hline \hline
NQG \cite{du2017learning} & 91.45 & 90.11 & 60.70 & 94.62 & 0.233 & 0.282 & 4.473 & 4.738 \\
+ BeamSearch & 94.33 & 93.42 & 62.08 & 95.56 & 0.569 & 0.775 & 5.406 & 5.812 \\
+ Top-k Sampling & 94.33 & 93.42 & 62.08 & 95.56 & 0.569 & 0.775 & 5.406 & 5.812 \\
+ Nucleus Sampling  & 94.33 & 93.42 & 62.08 & 95.56 & 0.569 & 0.775 & 5.406 & 5.812 \\
\textbf{+ QPP (Ours)} & \textbf{96.82} & \textbf{96.33} & \textbf{64.38} & \textbf{97.49} & \textbf{3.177} & \textbf{5.289} & \textbf{7.100} & \textbf{7.777} \\ \hline\hline
NQG++ \cite{zhou2017neural} & 97.11 & 96.65 & 71.57 & 97.86 & 0.229 & 0.275 & 4.419 & 4.648 \\
+ BeamSearch & 98.35 & 98.07 & 72.98 & 98.55 & 0.618 & 0.848 & 5.497 & 5.953 \\
+ Top-k Sampling & 94.33 & 93.42 & 62.08 & 95.56 & 0.569 & 0.775 & 5.406 & 5.812 \\
+ Nucleus Sampling  & 94.33 & 93.42 & 62.08 & 95.56 & 0.569 & 0.775 & 5.406 & 5.812 \\
\textbf{+ QPP (Ours)} & {\textbf{99.15}} & {\textbf{99.03}} & {\textbf{74.01}} & {\textbf{99.11}} & \textbf{3.183} &  \textbf{5.293} & \textbf{7.111} & \textbf{7.798} \\ \hline\hline
BERT-SQG \cite{chan2019recurrent} & 89.07 & 87.99 & 65.25 & 94.91 & 0.228 & 0.276 & 4.594 & 4.849 \\
+ BeamSearch &95.45   &94.84  &66.39  &96.22  &0.510  &0.713  &5.522  &6.015  \\
+ Top-k Sampling & 94.33 & 93.42 & 62.08 & 95.56 & 0.569 & 0.775 & 5.406 & 5.812 \\
+ Nucleus Sampling  & 94.33 & 93.42 & 62.08 & 95.56 & 0.569 & 0.775 & 5.406 & 5.812 \\
\textbf{+ QPP (Ours)} & \textbf{96.54} & \textbf{96.19} & \textbf{67.51} & \textbf{97.42} & {\textbf{3.344}} &{\textbf{5.332}} & {\textbf{7.173}} & {\textbf{7.816}} \\ \hline
\end{tabular}%
\end{table*}


==> Tables/table3.tex <==
\begin{table*}[t]
\centering
\caption{The performance on MIMIC-III test set of two QA models: DocReader and ClinicalBERT that are trained based on different QA corpora. emrQA is also included as a baseline dataset to help illustrate the generated diverse questions on MIMIC-III are useful to improve the QA model performance on new contexts.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccc|cccc}
\hline
\multirow{3}{*}{\textbf{QA Datasets}} & \multicolumn{4}{c|}{\textbf{DocReader}} & \multicolumn{4}{c}{\textbf{ClinicalBERT}} \\ \cline{2-9} 
 & \multicolumn{2}{c}{\textbf{Dev}} & \multicolumn{2}{c|}{\textbf{Test}} & \multicolumn{2}{c}{\textbf{Dev}} & \multicolumn{2}{c}{\textbf{Test}} \\ \cline{2-9} 
 & \textbf{EM} & \textbf{F1} & \textbf{EM} & \textbf{F1} & \textbf{EM} & \textbf{F1} & \textbf{EM} & \textbf{F1} \\ \hline
emrQA \cite{pampari2018emrqa} & 58.41 & 80.48 & 63.48 & 79.99 & 58.73 & 77.58 & 63.17 & 79.59 \\ \hline
NQG Generated \cite{du2017learning} & 62.52 & 80.05 & 64.96 & 79.15 & 58.23 & 77.33 & 61.38 & 78.11 \\
+ BeamSearch & 64.60 & 81.65 & 68.07 & 81.66 & 61.28 & 80.28 & 64.80 & 80.34 \\
\textbf{+ QuesPhrase (Ours)} & \textbf{67.24} & \textbf{84.46} & \textbf{70.09} & \textbf{83.44} & \textbf{64.47} & \textbf{82.70} & \textbf{65.89} & \textbf{80.88} \\ \hline
NQG++ Generated \cite{zhou2017neural} & 62.82 & 79.88 & 66.04 & 79.35 & 57.97 & 76.71 & 60.92 & 76.88 \\
+ BeamSearch & 64.91 & 81.49 & 69.08 & 81.18 & 60.40 & 79.61 & 65.50 & 80.83 \\
\textbf{+ QuesPhrase (Ours)} & \textbf{67.41} & \textbf{84.25} & \textbf{71.10} & \textbf{84.06} & \textbf{63.16} & \textbf{81.16} & \textbf{66.67} & \textbf{81.88} \\ \hline
BERT-SQG Generated \cite{chan2019recurrent} & 62.59 & 80.49 & 64.10 & 78.26 & 58.20 & 76.69 & 60.92 & 79.05 \\
+ BeamSearch & 64.54 & 82.02 & 67.91 & 81.27 & 61.88 & 81.17 & 63.25 & 79.88 \\
\textbf{+ QuesPhrase (Ours)} & \textbf{67.42} & \textbf{84.55} & \textbf{69.47} & \textbf{83.80} & \textbf{65.38} & \textbf{82.69} & \textbf{64.49} & \textbf{80.92} \\ \hline
\end{tabular}%
}
\label{tbl:qa_results}
\end{table*}


==> Tables/table4.tex <==
\begin{table}[t]
\centering
\caption{Impact of question phrase length ($l$) on QG model performance (on emrQA dev set). }
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\hline
\multirow{2}{*}{Models} & \multicolumn{2}{c}{\textbf{Relevance}} & \multicolumn{2}{c}{\textbf{Diversity}} \\ \cline{2-5} 
 & \multicolumn{1}{l}{\textbf{BLEU4}} & \multicolumn{1}{l}{\textbf{METEOR}} & \multicolumn{1}{l}{\textbf{Distinct4}} & \multicolumn{1}{l}{\textbf{Entropy4}} \\ \hline
NQG++ & 97.36 & 72.52 & 0.313 & 4.779 \\
+QPP ($l$=1) & 99.08 & 72.67 & 2.228 & 7.092 \\
+QPP ($l$=2) & \textbf{99.10} & \textbf{74.51} & \textbf{5.554} & 7.801 \\
+QPP ($l$=3) & \textbf{99.10} & 73.58 & 5.157 & \textbf{8.026} \\ \hline
% GT & / & / & 16.777 & 8.542 \\ \hline
\end{tabular}%
}
\label{tbl:ablation}
% \vspace{-10pt}
\end{table}


==> Tables/tableA1.tex <==
\begin{table*}[t!]
\centering
\caption{Distributions of the generated questions of different models and the ground truth in the emrQA dataset. QPP: Question Phrase Prediction; KL: Kullback–Leibler divergence. All numbers are percentages.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccc|c}
\hline
Models & \textbf{What} & \textbf{When} & \textbf{Has} & \textbf{Was} & \textbf{Why} & \textbf{How} & \textbf{Is} & \textbf{Did} & \textbf{Can} & \textbf{Any} & \textbf{Does} &  \textbf{\begin{tabular}[c]{@{}c@{}}KL\\ (Gen$||$GT)\end{tabular}} \\ \hline
NQG & 0.00 & 0.00 & 3.95 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 96.05 & 84.2 \\
+BeamSearch & 29.94 & 0.00 & 5.54 & 0.00 & 0.00 & 0.00 & 1.38 & 0.00 & 0.00 & 0.00 & 63.14 & 45.2 \\
\textbf{+QPP (Ours)} & 8.39 & 0.01 & 25.37 & 4.44 & 0.91 & 0.87 & 9.09 & 0.27 & 4.03 & 12.72 & 33.89 & \textbf{11.0} \\ \hline
NQG++ & 0.09 & 0.00 & 3.53 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 96.28 & 84.3 \\
+BeamSearch & 44.04 & 0.00 & 0.09 & 0.00 & 0.00 & 0.22 & 2.01 & 0.00 & 0.00 & 0.00 & 53.64 & 66.4 \\
\textbf{+QPP (Ours)} & 8.09 & 0.01 & 25.54 & 4.42 & 0.75 & 0.81 & 9.16 & 0.23 & 4.05 & 12.80 & 34.13 & \textbf{11.2} \\ \hline
BERT-SQG & 0.72 & 0.00 & 6.32 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 92.96 & 74.5 \\
+BeamSearch & 29.31 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 25.05 & 0.00 & 0.00 & 0.00 & 45.62 & 47.4  \\
\textbf{+QPP (Ours)} & 8.01 & 0.01 & 25.56 & 4.44 & 0.82 & 0.80 & 9.17 & 0.25 & 4.05 & 12.74 & 34.16 & \textbf{11.2} \\ \hline
GT & 13.80 & 0.01 & 26.73 & 1.94 & 0.63 & 1.16 & 13.24 & 0.14 & 1.31 & 4.11 & 36.93 & - \\ \hline
\end{tabular}%
}
\vspace{-10pt}
\label{tbl:ques_distribution}
\end{table*}


==> Tables/tableA2.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcc}
\hline
 & QPP acc & QG acc \\ \hline
NQG & / & 74.32 \\
NQG++ & / & 74.54 \\
BERT-SQG & / & 79.78 \\ \hline
QPP-NQG & 99.2 & 85.15 \\
QPP-NQG++ & 99.17 & 85.27 \\
QPP-BERT-SQG & 99.19 & 88.15 \\ \hline
\end{tabular}
\caption{QPP and QG performance on dev set in terms of per-token accuracy. All numbers are percentages.}
\label{dev_qg}
\end{table}

==> Tables/tableA3.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
\model & QG & QA & overall \\ \hline
NQG\&DocReader & 6 & 17 & 24.5 \\
NQG++\&DocReader & 7.5 & 20 & 29 \\
BERT-SQG\&DocReader & 13 & 18 & 32.5 \\
NQG\&CliniBERT & 6 & 3.5 & 11 \\
NQG++\&CliniBERT & 7.5 & 4 & 13 \\
BERT-SQG\&CliniBERT & 13.5 & 3.5 & 18.5 \\ \hline
\end{tabular}}
\caption{The running time (hour) of QPP-augmented QG, QA and overall \model based on our selected QG \& QA combinations}
\label{run_time}
\end{table}

==> Tables/tableA4.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcc}
\hline
Parameter & Search Trials & Best \\ \hline
Dropout & {[}0.3,0.45,0.6,0.75,0.9{]} & 0.75 \\
LSTM Layers & {[}1,2,3,4{]} & 3 \\
QP Length & {[}1,2,3{]} & 2 \\ \hline
\end{tabular}
\caption{Hyperparameter searches for Question Phrase Prediction (QPP) Module}
\label{QPP_tune}
\end{table}


==> Tables/tableA5.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcc}
\hline
Parameter & Search Trials & Best \\ \hline
length ($\eta$) & {[}1,3,5,10{]} & 3 \\
distance ($\gamma$) & {[}1,3,5,10{]} & 3 \\ \hline
\end{tabular}
\caption{Hyperparameter searches for \textit{``merge-and-drop"} method}
\label{AEE_tune}
\end{table}

==> Tables/tableA6.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccccc}
\hline
& \textbf{does} & \textbf{has} & \textbf{what} & \textbf{is} & \textbf{any} & \textbf{was} & \textbf{can} & \textbf{how} & \textbf{why} & \textbf{when} & \textbf{did} & \textbf{have} & \textbf{were}  \\ \hline
\textbf{human-verified} & 28.00 & 22.05 & 18.77 & 10.15 & 7.18 & 5.44 & 4.62 & 2.15 & 0.92 & 0.31 & 0.31 & 0.00 & 0.10 \\
\textbf{human-generated} & 25.00 & 10.90 & 16.67 & 8.01 & 7.05 & 4.17 & 2.24 & 6.41 & 9.62 & 5.77 & 3.85 & 0.32 & 0.00 \\
\textbf{overall test} & 27.27 & 19.35 & 18.26 & 9.63 & 7.15 & 5.13 & 4.04 & 3.19 & 3.03 & 1.63 & 1.17 & 0.08 & 0.08\\ \hline
\end{tabular}%
}
\caption{Distributions of question types in the test dataset. All numbers are percentages.}
\label{tbl:ques_test_distribution}
\end{table*}


==> figure.tex <==


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{Figures/QA&QG_Task.pdf}
%     \caption{Illustration of QA and QG task.}
%     \label{fig:qa_qg_task}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{Figures/QA&QG_Task2.pdf}
    \caption{Illustration of QA and QG task.}
    \label{fig:qa_qg_task}
\end{figure}


